Nuance Matters: Probing Epistemic Consistency in Causal Reasoning

To address this gap, our study introduces the concept of causal epistemic consistency, which focuses on the self-consistency of Large Language Models (LLMs) in differentiating intermediates with nuanced differences in causal reasoning. We propose a suite of novel metrics -- intensity ranking concordance, cross-group position agreement, and intra-group clustering -- to evaluate LLMs on this front. Through extensive empirical studies on 21 high-profile LLMs, including GPT-4, Claude3, and LLaMA3-70B, we have favoring evidence that current models struggle to maintain epistemic consistency in identifying the polarity and intensity of intermediates in causal reasoning. Additionally, we explore the potential of using internal token probabilities as an auxiliary tool to maintain causal epistemic consistency. In summary, our study bridges a critical gap in AI research by investigating the self-consistency over fine-grained intermediates involved in causal reasoning.

==> appendices/checklist.tex <==
This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) yes
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) yes
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) yes

\end{itemize}



\noindent Does this paper make theoretical contributions? (yes/no) yes
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no) yes
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no) yes
    \item Proofs of all novel claims are included. (yes/partial/no) yes
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no) yes
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no) yes
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA) yes
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA) yes
\end{itemize}


\noindent Does this paper rely on one or more datasets? (yes/no) yes

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) yes
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) yes
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) yes
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) yes
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) yes
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) yes
\end{itemize}

\noindent Does this paper include computational experiments? (yes/no) yes

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no) yes
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) yes
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) yes
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) yes
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) yes
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) yes
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) yes
    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no) yes
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) yes
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) yes
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) yes
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) yes
\end{itemize}


==> appendices/full-generations.tex <==
In addition, we experimented with generating all ten fine-grained intermediates given only the cause and effect pair. The prompt used for such generation can be found in Figure~\ref{fig:prompt_intermediate_generation}. The evaluations of the full generation dataset could be found in Table~\ref{tab:full_gpt_results_with_generating_10_arguments}




\begin{figure*}[htb]
    \centering\input{figures/prompts/full_intermediate_generation}
    \caption{Prompts for generating full fine-grained intermediates with LLMs. The \variableP{\{argument\_type\}} are selected from \{defeater, supporters\}. The \variableP{\{strength\}} are selected from \{stronger, weakener\}. }
    \label{fig:prompt_intermediate_generation}
\end{figure*}

\begin{table*}[htp!]
    \centering
    \input{figures/table_minipages/appendix_metrics}
    \caption{Comparison of different LLMs’ causal epistemic consistency on discerning fine-grained intermediates in causality on the full generation intermediates dataset.}
    \label{tab:full_gpt_results_with_generating_10_arguments}
\end{table*}

==> appendices/open-source.tex <==
\subsection{Generation}
In zero-shot settings, open-source models often struggle to produce text in a specific format consistently. This inconsistency requires steering the models towards generating easily extractable text using the same set of rules each time (e.g., find the lines that start with '1.' or '2.').
\subsection{Ranking}
Similarly, we provide separate scripts for the ranking component. In this part, the models rank the 10 arguments in different ways. For instance, some models output the ranking on a single line, while others insert a line break between each number. Therefore, the primary challenge lies in extracting the ranking correctly.

==> figures/illustration/fine-grained-da.tex <==
\begin{tikzpicture}

% Create the color gradient
\shade[left color=deepskyblue4, right color=darkorange, middle color=white] (0,0) rectangle (10,2);

\node at (1, 1) {$d_n$};
\node at (2, 1) {$d_{n-1}$};
\node at (4, 1) {$d_1$};

\node at (5, 1.5) {$(C, E)$};

\node at (6, 1) {$a_1$};
\node at (7, 1) {$a_2$};
\node at (9, 1) {$a_n$};

\node at (9, 1) {$a_n$};


\end{tikzpicture}

==> figures/illustration/illustration.tex <==
% Gradient Info
  
\tikzset {_t8qahukpi/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_lh8b6bhur}{150bp}{rgb(0bp)=(0.27,0.51,0.71);
rgb(37.5bp)=(0.27,0.51,0.71);
rgb(37.5bp)=(0.27,0.51,0.71);
rgb(50bp)=(1,1,1);
rgb(62.5bp)=(1,0.5,0);
rgb(100bp)=(1,0.5,0)}
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,187); %set diagram left start at 0, and has height of 187

%Straight Lines [id:da2250737242176215] 
\draw    (53,53) -- (221,53) ;
\draw [shift={(223,53)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Square [id:dp4552601648394119] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][fill={rgb, 255:red, 70; green, 130; blue, 180 }  ,fill opacity=1 ] (63,68) -- (73,68) -- (73,78) -- (63,78) -- cycle ;
%Shape: Square [id:dp6023152376943834] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][fill={rgb, 255:red, 164; green, 194; blue, 218 }  ,fill opacity=1 ] (83,68) -- (93,68) -- (93,78) -- (83,78) -- cycle ;
%Shape: Square [id:dp6406241488424533] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][fill={rgb, 255:red, 118; green, 163; blue, 200 }  ,fill opacity=1 ] (103,68) -- (113,68) -- (113,78) -- (103,78) -- cycle ;
%Shape: Circle [id:dp6005048641878084] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 222; blue, 190 }  ,fill opacity=1 ] (123,73) .. controls (123,70.24) and (125.24,68) .. (128,68) .. controls (130.76,68) and (133,70.24) .. (133,73) .. controls (133,75.76) and (130.76,78) .. (128,78) .. controls (125.24,78) and (123,75.76) .. (123,73) -- cycle ;
%Shape: Square [id:dp4267635085997419] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][fill={rgb, 255:red, 211; green, 226; blue, 237 }  ,fill opacity=1 ] (143,68) -- (153,68) -- (153,78) -- (143,78) -- cycle ;
%Shape: Circle [id:dp4096774529953562] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 156; blue, 59 }  ,fill opacity=1 ] (163,73) .. controls (163,70.24) and (165.24,68) .. (168,68) .. controls (170.76,68) and (173,70.24) .. (173,73) .. controls (173,75.76) and (170.76,78) .. (168,78) .. controls (165.24,78) and (163,75.76) .. (163,73) -- cycle ;
%Shape: Circle [id:dp1919094575708804] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 189; blue, 124 }  ,fill opacity=1 ] (183,73) .. controls (183,70.24) and (185.24,68) .. (188,68) .. controls (190.76,68) and (193,70.24) .. (193,73) .. controls (193,75.76) and (190.76,78) .. (188,78) .. controls (185.24,78) and (183,75.76) .. (183,73) -- cycle ;
%Shape: Circle [id:dp011937431520289365] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 127; blue, 0 }  ,fill opacity=1 ] (203,73) .. controls (203,70.24) and (205.24,68) .. (208,68) .. controls (210.76,68) and (213,70.24) .. (213,73) .. controls (213,75.76) and (210.76,78) .. (208,78) .. controls (205.24,78) and (203,75.76) .. (203,73) -- cycle ;
%Shape: Square [id:dp5577346964548757] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ] (63,128) -- (73,128) -- (73,138) -- (63,138) -- cycle ;
%Shape: Square [id:dp8276042673713062] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ] (83,128) -- (93,128) -- (93,138) -- (83,138) -- cycle ;
%Shape: Square [id:dp08154955970926525] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ] (103,128) -- (113,128) -- (113,138) -- (103,138) -- cycle ;
%Shape: Circle [id:dp7075609500159628] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ] (123,133) .. controls (123,130.24) and (125.24,128) .. (128,128) .. controls (130.76,128) and (133,130.24) .. (133,133) .. controls (133,135.76) and (130.76,138) .. (128,138) .. controls (125.24,138) and (123,135.76) .. (123,133) -- cycle ;
%Shape: Square [id:dp7079730131648643] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ] (143,128) -- (153,128) -- (153,138) -- (143,138) -- cycle ;
%Shape: Circle [id:dp4226469305241962] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ] (163,133) .. controls (163,130.24) and (165.24,128) .. (168,128) .. controls (170.76,128) and (173,130.24) .. (173,133) .. controls (173,135.76) and (170.76,138) .. (168,138) .. controls (165.24,138) and (163,135.76) .. (163,133) -- cycle ;
%Shape: Circle [id:dp4438955377197631] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ] (183,133) .. controls (183,130.24) and (185.24,128) .. (188,128) .. controls (190.76,128) and (193,130.24) .. (193,133) .. controls (193,135.76) and (190.76,138) .. (188,138) .. controls (185.24,138) and (183,135.76) .. (183,133) -- cycle ;
%Shape: Circle [id:dp7072172950093576] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ] (203,133) .. controls (203,130.24) and (205.24,128) .. (208,128) .. controls (210.76,128) and (213,130.24) .. (213,133) .. controls (213,135.76) and (210.76,138) .. (208,138) .. controls (205.24,138) and (203,135.76) .. (203,133) -- cycle ;
%Shape: Square [id:dp11539546563320902] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ] (63,158) -- (73,158) -- (73,168) -- (63,168) -- cycle ;
%Shape: Square [id:dp5266059363268061] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ] (83,158) -- (93,158) -- (93,168) -- (83,168) -- cycle ;
%Shape: Square [id:dp8210150345319975] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ] (103,158) -- (113,158) -- (113,168) -- (103,168) -- cycle ;
%Shape: Circle [id:dp9305367147719761] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ] (123,163) .. controls (123,160.24) and (125.24,158) .. (128,158) .. controls (130.76,158) and (133,160.24) .. (133,163) .. controls (133,165.76) and (130.76,168) .. (128,168) .. controls (125.24,168) and (123,165.76) .. (123,163) -- cycle ;
%Shape: Square [id:dp6736677365494113] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ] (143,158) -- (153,158) -- (153,168) -- (143,168) -- cycle ;
%Shape: Circle [id:dp6941099110769409] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ] (163,163) .. controls (163,160.24) and (165.24,158) .. (168,158) .. controls (170.76,158) and (173,160.24) .. (173,163) .. controls (173,165.76) and (170.76,168) .. (168,168) .. controls (165.24,168) and (163,165.76) .. (163,163) -- cycle ;
%Shape: Circle [id:dp9239751032109631] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ] (183,163) .. controls (183,160.24) and (185.24,158) .. (188,158) .. controls (190.76,158) and (193,160.24) .. (193,163) .. controls (193,165.76) and (190.76,168) .. (188,168) .. controls (185.24,168) and (183,165.76) .. (183,163) -- cycle ;
%Shape: Circle [id:dp9778111760560215] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ] (203,163) .. controls (203,160.24) and (205.24,158) .. (208,158) .. controls (210.76,158) and (213,160.24) .. (213,163) .. controls (213,165.76) and (210.76,168) .. (208,168) .. controls (205.24,168) and (203,165.76) .. (203,163) -- cycle ;
%Shape: Square [id:dp7388197204463267] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][fill={rgb, 255:red, 70; green, 130; blue, 180 }  ,fill opacity=1 ] (63,98) -- (73,98) -- (73,108) -- (63,108) -- cycle ;
%Shape: Square [id:dp36430745238589246] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][fill={rgb, 255:red, 164; green, 194; blue, 218 }  ,fill opacity=1 ] (83,98) -- (93,98) -- (93,108) -- (83,108) -- cycle ;
%Shape: Square [id:dp9843183884444271] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][fill={rgb, 255:red, 118; green, 163; blue, 200 }  ,fill opacity=1 ] (103,98) -- (113,98) -- (113,108) -- (103,108) -- cycle ;
%Shape: Circle [id:dp21937747233874005] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 222; blue, 190 }  ,fill opacity=1 ] (123,103) .. controls (123,100.24) and (125.24,98) .. (128,98) .. controls (130.76,98) and (133,100.24) .. (133,103) .. controls (133,105.76) and (130.76,108) .. (128,108) .. controls (125.24,108) and (123,105.76) .. (123,103) -- cycle ;
%Shape: Square [id:dp6803757464370945] 
\draw  [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][fill={rgb, 255:red, 211; green, 226; blue, 237 }  ,fill opacity=1 ] (143,98) -- (153,98) -- (153,108) -- (143,108) -- cycle ;
%Shape: Circle [id:dp9602541196354084] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 156; blue, 59 }  ,fill opacity=1 ] (163,103) .. controls (163,100.24) and (165.24,98) .. (168,98) .. controls (170.76,98) and (173,100.24) .. (173,103) .. controls (173,105.76) and (170.76,108) .. (168,108) .. controls (165.24,108) and (163,105.76) .. (163,103) -- cycle ;
%Shape: Circle [id:dp01203958360388957] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 189; blue, 124 }  ,fill opacity=1 ] (183,103) .. controls (183,100.24) and (185.24,98) .. (188,98) .. controls (190.76,98) and (193,100.24) .. (193,103) .. controls (193,105.76) and (190.76,108) .. (188,108) .. controls (185.24,108) and (183,105.76) .. (183,103) -- cycle ;
%Shape: Circle [id:dp09180937766833219] 
\draw  [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 127; blue, 0 }  ,fill opacity=1 ] (203,103) .. controls (203,100.24) and (205.24,98) .. (208,98) .. controls (210.76,98) and (213,100.24) .. (213,103) .. controls (213,105.76) and (210.76,108) .. (208,108) .. controls (205.24,108) and (203,105.76) .. (203,103) -- cycle ;
%Rounded Rect [id:dp2550913658565259] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (80,98.7) .. controls (80,96.93) and (81.43,95.5) .. (83.2,95.5) -- (112.8,95.5) .. controls (114.57,95.5) and (116,96.93) .. (116,98.7) -- (116,108.3) .. controls (116,110.07) and (114.57,111.5) .. (112.8,111.5) -- (83.2,111.5) .. controls (81.43,111.5) and (80,110.07) .. (80,108.3) -- cycle ;
%Rounded Rect [id:dp15627398881996868] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (120,98.7) .. controls (120,96.93) and (121.43,95.5) .. (123.2,95.5) -- (152.8,95.5) .. controls (154.57,95.5) and (156,96.93) .. (156,98.7) -- (156,108.3) .. controls (156,110.07) and (154.57,111.5) .. (152.8,111.5) -- (123.2,111.5) .. controls (121.43,111.5) and (120,110.07) .. (120,108.3) -- cycle ;
%Rounded Rect [id:dp015361658963946923] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (160,98.7) .. controls (160,96.93) and (161.43,95.5) .. (163.2,95.5) -- (192.8,95.5) .. controls (194.57,95.5) and (196,96.93) .. (196,98.7) -- (196,108.3) .. controls (196,110.07) and (194.57,111.5) .. (192.8,111.5) -- (163.2,111.5) .. controls (161.43,111.5) and (160,110.07) .. (160,108.3) -- cycle ;
%Rounded Rect [id:dp9345629617468274] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (120,128.7) .. controls (120,126.93) and (121.43,125.5) .. (123.2,125.5) -- (152.8,125.5) .. controls (154.57,125.5) and (156,126.93) .. (156,128.7) -- (156,138.3) .. controls (156,140.07) and (154.57,141.5) .. (152.8,141.5) -- (123.2,141.5) .. controls (121.43,141.5) and (120,140.07) .. (120,138.3) -- cycle ;
%Straight Lines [id:da5230097563896141] 
\draw [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][line width=0.75]    (68,173) -- (88,173) ;
\draw [shift={(88,173)}, rotate = 180] [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][line width=0.75]    (0,2.24) -- (0,-2.24)   ;
\draw [shift={(68,173)}, rotate = 180] [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][line width=0.75]    (0,2.24) -- (0,-2.24)   ;
%Straight Lines [id:da08238782024707691] 
\draw [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][line width=0.75]    (108,173) -- (148,173) ;
\draw [shift={(148,173)}, rotate = 180] [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][line width=0.75]    (0,2.24) -- (0,-2.24)   ;
\draw [shift={(108,173)}, rotate = 180] [color={rgb, 255:red, 70; green, 130; blue, 180 }  ,draw opacity=1 ][line width=0.75]    (0,2.24) -- (0,-2.24)   ;
%Straight Lines [id:da02970316375620663] 
\draw [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (188,153) -- (208,153) ;
\draw [shift={(208,153)}, rotate = 180] [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (0,2.24) -- (0,-2.24)   ;
\draw [shift={(188,153)}, rotate = 180] [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (0,2.24) -- (0,-2.24)   ;
%Straight Lines [id:da10516853912901158] 
\draw [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (128,153) -- (168,153) ;
\draw [shift={(168,153)}, rotate = 180] [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (0,2.24) -- (0,-2.24)   ;
\draw [shift={(128,153)}, rotate = 180] [color={rgb, 255:red, 255; green, 127; blue, 0 }  ,draw opacity=1 ][line width=0.75]    (0,2.24) -- (0,-2.24)   ;
%Shape: Rectangle [id:dp19992844587414393] 
\path  [shading=_lh8b6bhur,_t8qahukpi] (230,45) -- (409.67,45) -- (409.67,63.75) -- (230,63.75) -- cycle ; % for fading 
 \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0 ] (230,45) -- (409.67,45) -- (409.67,63.75) -- (230,63.75) -- cycle ; % for border 


% Text Node
\draw (57,22.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{28.92pt}\setlength\topsep{0pt}
\begin{center}
Low\\
Ranking
\end{center}

\end{minipage}};
% Text Node
\draw (163.5,22.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{28.92pt}\setlength\topsep{0pt}
\begin{center}
High\\
Ranking
\end{center}

\end{minipage}};
% Text Node
\draw (8,57) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{28.92pt}\setlength\topsep{0pt}
\begin{center}
LLM's\\
Ranking
\end{center}

\end{minipage}};
% Text Node
\draw (8,98.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{29.71pt}\setlength\topsep{0pt}
\begin{center}
Intensity
\end{center}

\end{minipage}};
% Text Node
\draw (1.5,128.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] 
{\begin{minipage}[lt]{37.65pt}\setlength\topsep{0pt}
\begin{center}
Direction
\end{center}

\end{minipage}};
% Text Node
\draw (1.5,158.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{37.65pt}\setlength\topsep{0pt}
\begin{center}
Clustering
\end{center}

\end{minipage}};
% Text Node
\draw (133.5,107.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny ❌}};
% Text Node
\draw (173.5,107.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny ❌}};
% Text Node
\draw (93.5,107.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny ❌}};
% Text Node
\draw (133.5,137.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\tiny ❌}};
% Text Node
\draw (68,176) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 70; green, 130; blue, 180 }  ,opacity=1 ] [align=left] {Close};
% Text Node
\draw (121.5,176) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 70; green, 130; blue, 180 }  ,opacity=1 ] [align=left] {Far};
% Text Node
\draw (141.5,143.5) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 70; green, 130; blue, 180 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{1,0.5,0}{Far}};
% Text Node
\draw (188,143.5) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 70; green, 130; blue, 180 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{1,0.5,0}{Close}};
% Text Node
\draw (230.33,18.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] 
{\begin{minipage}[lt]{51.14pt}\setlength\topsep{0pt}
\begin{center}
Low\\Actual Intensity
\end{center}

\end{minipage}};
% Text Node
\draw (335.33,18.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{51.14pt}\setlength\topsep{0pt}
\begin{center}
High\\Actual Intensity
\end{center}

\end{minipage}};
% Text Node
\draw (234.33,96.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont {\scriptsize \textit{The one with higher ranking in the pair }}}\\[-5pt]{\fontfamily{ptm}\selectfont {\scriptsize \textit{should have a higher actual intensity.}}}};
% Text Node
\draw (234.83,126.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize {\fontfamily{ptm}\selectfont \textit{Each \textcolor[rgb]{1,0.5,0}{supporter element} should have a }}}\\[-5pt]{\scriptsize {\fontfamily{ptm}\selectfont \textit{higher ranking than each \textcolor[rgb]{0.27,0.51,0.71}{defeating element}.}}}};
% Text Node
\draw (234.83,156) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont {\scriptsize \textit{Within each group, the elements should be}}}\\[-5pt]{\scriptsize {\fontfamily{ptm}\selectfont \textit{clustered closely.}}}};


\end{tikzpicture}


==> figures/illustration/intro_example_consistency.tex <==
\newcommand{\chatgptemoji}{\raisebox{-2pt}{\includegraphics[width=1.0em]{figures/icons/chatgpt.png}}\xspace}
\newcommand{\llamaemoji}{\raisebox{-1pt}{\includegraphics[width=1.0em]{figures/icons/meta-llama-symbol.png}}\xspace}

\usetikzlibrary{shapes.geometric}

\definecolor{sColor}{RGB}{255,140,0}  % Darker orange
\definecolor{dColor}{RGB}{70,130,180}   % Steel blue


\usetikzlibrary{arrows.meta, positioning, shadows, fit, backgrounds}
\definecolor{steelblue}{RGB}{70,130,180}
\definecolor{highSupport}{RGB}{255,140,0}  % Darker orange
\definecolor{mediumSupport}{RGB}{255,165,0} % Standard orange
\definecolor{lowSupport}{RGB}{255,200,150}  % Light orange
\definecolor{highOppose}{RGB}{70,130,180}   % Steel blue
\definecolor{mediumOppose}{RGB}{135,206,235} % Sky blue
\definecolor{lowOppose}{RGB}{176,224,230}   % Powder blue

\definecolor{darkgreen}{HTML}{008000}
\definecolor{darkblue}{HTML}{0000FF}
\definecolor{darkgray}{HTML}{808080}

% Define the custom style
\tikzset{
  customnode/.style={
    rectangle, fill=white, draw, rounded corners, 
    text width=12cm, minimum height=6em, inner sep=0em,
    font=\large, align=left,
  },
  topbar1/.style={
    rectangle, fill=#1, minimum height=0.4cm, anchor=north west,
  },
  topbar2/.style={
    rectangle, fill=#1!20, minimum height=0.4cm, anchor=north west,
  },
  bigcircle/.style={
    circle, fill=#1, text centered, minimum size=2cm, font=\large\bfseries, text=white,
  },
  title/.style={
    font=\bfseries\huge, anchor=west,
  },
  sectionNode/.style = {
    rectangle,
    draw,
    align=center,
    rounded corners,
    minimum height=2em,
    minimum width=5em,
    fill=#1
    },
}

\makeatletter
\pgfdeclareshape{big arrow}{
    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{south east}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{north east}
    \backgroundpath{
        % Draw the arrow shape
        \def\arrowhead{0.3} % width of the arrowhead
        \def\arrowlength{0.5} % length of the arrowhead
        \def\halfheight{0.2} % half the height of the arrow body
        \path[fill=black] 
        (-0.5, \halfheight) -- (\arrowlength-0.5, \halfheight) -- (\arrowlength-0.5, \arrowhead) -- (0.5, 0) -- (\arrowlength-0.5, -\arrowhead) -- (\arrowlength-0.5, -\halfheight) -- (-0.5, -\halfheight) -- cycle;
    }
}
\makeatother


% Define the custom node macro
\newcommand{\customnode}[6]{
    % Define styles
    \tikzstyle{block} = [rectangle, text width=4.5cm, rounded corners, inner sep=1em]
    \tikzstyle{bigcircle} = [circle, fill=#1, text centered, minimum size=0.75cm, font=\large\bfseries, text=white]
    \tikzstyle{title} = [font=\bfseries\large, anchor=west]
    \tikzstyle{topbar1} = [rectangle, fill=#1, minimum height=0.4cm, anchor=north west]
    \tikzstyle{topbar2} = [rectangle, fill=#1!20, minimum height=0.4cm, anchor=north west]

    \begin{scope}[shift={(#5,#6)}]
        % Draw the top bars
        \node[topbar1, minimum width=1cm] (topbar1) at (0,0) {};
        \node[topbar2, minimum width=4cm, right=0cm of topbar1.east] (topbar2) {};

        % Draw the circle
        \node[bigcircle, anchor=north] (numberCircle) at ([xshift=0cm,yshift=-0.5cm] topbar1.south) {\huge #2};

        % Draw the title
        \node[title, anchor=west] at ([xshift=0.25cm, yshift=0cm] numberCircle.east) {\huge #3};

        % Draw the block
        \node[block, below=0.2cm of numberCircle, anchor=north west, align=left, xshift=-0.5cm, yshift=0.5cm] (block) {#4
            % \begin{minipage}{4.5cm}
            %     #4
            % \end{minipage}
        };
    \end{scope}
}


\begin{tikzpicture}[
    node distance=2cm,
    auto,
    thick,
    text node/.style={font=\sffamily\Large\bfseries, align=center, minimum size=1.5cm},
    ce node/.style={rectangle, align=center, minimum height=2cm, text width=7cm, font=\sffamily, rounded corners},
    intermediate node/.style={rectangle, align=center, minimum height=3.0cm, text width=17cm, font=\sffamily, rounded corners},
    supporter node/.style={rectangle, align=center, minimum height=1cm, text width=6cm, font=\sffamily\huge, rounded corners},
    defeater node/.style={rectangle, align=center, minimum height=1cm, text width=6cm, font=\sffamily, rounded corners},
    text node/.style={rectangle, align=left, minimum height=1cm, text width=17cm, font=\sffamily, rounded corners},
    gradient node/.style={rectangle, minimum width=0.5cm, minimum height=9cm, shading=axis, shading angle=0},
    line/.style={-Latex, thick}
    ]

    \node[ce node, fill=gray!30] (cause) at (3.5, 5) {\Large The number of hours a student studies. };
    \node[ce node, fill=gray!30] (effect) at (13.5, 5) {\Large The score a student achieves on an exam.};

    
    \node[intermediate node, fill=gray!10] (intermediate) at (8.5, 1.8) {};
    \node[supporter node, fill=sColor!30] (lowSupport) at (4.0, 2.5) {A weak supporter}; 
    \node[supporter node, fill=sColor!80] (highSupport) at (4.0, 1.0) {A strong supporter}; 
    \node[defeater node, fill=dColor!30] (lowDefeat) at (13.0, 2.5) {A weak supporter}; 
    \node[defeater node, fill=dColor!80] (highDefeat) at (13.0, 1.0) {A strong supporter};     
    
    \node[text node, fill=white!10] (questionNode) at (8.5, -0.5) {\huge For these fine-grained intermediates, can LLMs~(\chatgptemoji, \llamaemoji) maintain causal epistemic consistency in discerning: };

    \customnode{darkgreen}{1}{Intensity}{\Large Which are stronger and which are weakener.}{0}{-1.5}
    \customnode{darkblue}{2}{Direction}{\Large Whether the intermediate is supporting or defeating.}{6}{-1.5}
    \customnode{orange}{3}{clustering}{which are stronger and which are weakener.}{12}{-1.5}

    % \draw[dotted, rounded corners=10pt] (-0.5,-3.5) rectangle (17.5,6.5);

    % \customnode{darkgreen}{1}{Intensity}{}{0}{-1}
    % \customnode{darkblue}{2}{Direction}{}{6}{-1}
    % \customnode{orange}{3}{clustering}{}{12}{-1}

    \draw[dotted, rounded corners=10pt] (-0.5,-4.5) rectangle (17.5,6.5);

    % \draw[line, line width=4mm] (cause) -- (effect);
    \node[big arrow, minimum width=10cm, minimum height=1cm, scale=1.2] at (8.5, 5) {};


    % draw lines
    \draw[dotted,line width=0.8mm] (-0.5,0.3) -- (17.5,0.3);
\end{tikzpicture}


==> figures/illustration/intro_example_finegrained.tex <==
\usetikzlibrary{arrows.meta, positioning, shadows, fit, backgrounds}
\definecolor{steelblue}{RGB}{70,130,180}
\definecolor{highSupport}{RGB}{255,140,0}  % Darker orange
\definecolor{mediumSupport}{RGB}{255,165,0} % Standard orange
\definecolor{lowSupport}{RGB}{255,200,150}  % Light orange
\definecolor{highOppose}{RGB}{70,130,180}   % Steel blue
\definecolor{mediumOppose}{RGB}{135,206,235} % Sky blue
\definecolor{lowOppose}{RGB}{176,224,230}   % Powder blue
\begin{tikzpicture}[
    node distance=2cm,
    auto,
    thick,
    text node/.style={font=\sffamily\Large\bfseries, align=center, minimum size=1.5cm},
    main node/.style={circle, draw, font=\sffamily\Large\bfseries, align=center, minimum size=4.5cm, drop shadow},
    support node/.style={rectangle, draw, fill=orange, text width=3cm, align=center, minimum height=2cm, font=\sffamily, drop shadow, rounded corners},
    oppose node/.style={rectangle, draw, fill=steelblue, text width=3cm, align=center, minimum height=2cm, font=\sffamily, drop shadow, rounded corners},
    bg node/.style={rectangle, align=center, minimum height=9cm, , text width=4cm, font=\sffamily, rounded corners},
    gradient node/.style={rectangle, minimum width=0.5cm, minimum height=9cm, shading=axis, shading angle=0},
    line/.style={-Latex, thick}
    ]

    \node[gradient node, bottom color=white, top color=highSupport] at (-8, 0) {}; % Left gradient bar for supporting
    \node[gradient node, bottom color=white, top color=highOppose] at (8, 0) {}; % Right gradient bar for opposing

    % Backgrounds for grouping
    \node[bg node, fill=steelblue!30] at (5.0, 0) {};
    \node[bg node, fill=orange!30] at (-5.0, 0) {};
    % Nodes
    \node[main node] (effect) at (0, 0) {};


    % Supporting intermediates
    \node[support node, fill=highSupport] (high) at (-5, 3) {Take an earlier train\\(Significant improvement)};
    \node[support node, fill=mediumSupport] (medium) at (-5, 0) {Arrive at the station in time\\(Moderate improvement)};
    \node[support node, fill=lowSupport] (low) at (-5, -3) {Check online that the train is running on time\\(Slight improvement)};

    % Opposing intermediates
    \node[oppose node, fill=highOppose] (highOpp) at (5, 3) {There is a strike of the railway personnel\\(Significantly negates effects)};
    \node[oppose node, fill=mediumOppose] (medOpp) at (5, 0) {The train breaks down on the way\\(Somewhat negates effects)};
    \node[oppose node, fill=lowOppose] (lowOpp) at (5, -3) {The train is running late\\(Minimally affects outcome)};


    % Lines
    \draw[line] (high) -- (effect);
    \draw[line] (medium) -- (effect);
    \draw[line] (low) -- (effect);
    \draw[line] (highOpp) -- (effect);
    \draw[line] (medOpp) -- (effect);
    \draw[line] (lowOpp) -- (effect);


    \definecolor{color1}{RGB}{255,100,100} % Light red
    \definecolor{color2}{RGB}{100,255,100} % Light green
    \definecolor{color3}{RGB}{100,100,255} % Light blue

    % Circle parameters
    \def\Radius{3cm}
    \coordinate (Center) at (0,0);

    % Scope for clipping
    \begin{scope}
    % Define colors
    \definecolor{topColor}{RGB}{255,150,150} % Light red
    \definecolor{middleColor}{RGB}{150,255,150} % Light green
    \definecolor{bottomColor}{RGB}{150,150,255} % Light blue

    % Define circle parameters
    \def\Radius{2.25cm}
    \coordinate (Center) at (0,0);

    % Define clipping path (only within the circle)
    \clip (Center) circle[radius=\Radius];

    % Calculate intersections of horizontal lines with the circle
    % y = +a and y = -a for some a < radius
    \pgfmathsetmacro{\a}{0.7} % Change this value to adjust the heights of the divisions

    % Draw and fill areas
    % Top area
    \fill[topColor] (Center) ++(-\Radius,\a) rectangle (\Radius,3);
    % Middle area
    \fill[middleColor] (Center) ++(-\Radius,\a) rectangle (\Radius,-\a);
    % Bottom area
    \fill[bottomColor] (Center) ++(-\Radius,-\a) rectangle (\Radius,-3);

    % Redraw the circle outline
    \draw[thick] (Center) circle[radius=\Radius];
    \end{scope}

    \node[text node] (effect) at (0, 0){Causation};
    \node[text node] (effect) at (0, 1.5){\small Take the  \\\small train to the airport};
    \node[text node] (effect) at (0, -1.5){\small Reach the flight \\\small in time};

\end{tikzpicture}

==> figures/prompts/full_intermediate_generation.tex <==
\begin{mdframed}[backgroundcolor=gray!20,linewidth=0pt] 
    \begin{framedwithtag}{Query template}{blue!30}{blue!10}{-45mm}{2mm}{%
    Generate ten arguments for the cause-effect relationship in which 
    
    `cause: \variableP{\{cause\}}' 
    
    leads to the occurrence of
    
    `effect: \variableP{\{effect\}}' 
    
    , without explanations, additional commentary, index or quotation marks. Of the ten arguments, five of them should support the causal pair, and five should defeat the causal pair. 
    In addition, the ten arguments should vary in their supporting or defeating strength. More specifically, the generation order should start from the strongest defeater, to the weakest defeater, to the weakest supporter, and lastly to the strongest supporter.  
    
    Please ensure that the generated arguments are around \variableP{\{avg\_len\_original\_args\}} words in length.  
    
    Make sure that there are no explanations or additional commentary for the output and that the generated arguments are separated by a new line character.
    }
    \end{framedwithtag}
    \vspace{-10mm}
    \begin{framedwithtag}{Example}{red!30}{red!10}{-10mm}{2mm}{%
    Generate ten arguments for the cause-effect relationship in which 
    
    `cause: Audiences are drawn to television shows that display real-world scenarios.' 
    
    leads to the occurrence of 
    
    `effect: Years later, Television dramas are among the most popular as individuals can relate to the characters.' 
    
    , without explanations, additional commentary, index or quotation marks. Of the ten arguments, five of them should support the causal pair, and five should defeat the causal pair. In addition, the ten arguments should vary in their supporting or defeating strength. More specifically, the generation order should start from the strongest defeater, to the weakest defeater, to the weakest supporter, and lastly to the strongest supporter. 
    
    Please ensure that the generated arguments are around 18 words in length. 
    
    Make sure that there are no explanations or additional commentary for the output and that the generated arguments are separated by a new line character.
    }
    \end{framedwithtag}
\end{mdframed} 

==> figures/table_minipages/metrics_comparison.tex <==
\newcommand{\midgrayline}[0]{\arrayrulecolor{gray!50}\midrule\arrayrulecolor{black}}
% \newcommand{\midgrayline}[0]{\midrule}
\def\columnComparisonWidth{4.6}
\def\fourColumnComparisonWidth{21.0}

\begin{tabular}{p{2cm}p{5.7 cm}p{\columnComparisonWidth cm}p{\columnComparisonWidth cm}p{\columnComparisonWidth cm}}
\toprule
\textbf{Aspect} & \shorttitle~(our work) & \textbf{Acronym Generation} & \textbf{Controllable Text Generation} & \textbf{Dual Text Generation} \\ 
\midrule
Objectives & Generating engaging headings consisting of \acronyms and \descriptions. & Generating acronyms for input text. & Generating text that meets specific constraints. & Generating two texts with dual dependency. \\ 
\midgrayline
Problem \quad definitions & $\{D \rightleftarrows A\} = f(X, \mathcal{M})$ & $ A = f(X)$ \;\; where $X$ is the input, $A$ is the expected acronym.  & $Y = f(X, \mathcal{M})$ \;\; where $X$ is the input while $M$ is the set of controlled elements.  & 
$
\begin{cases}
    Y = f(X) \\
    X = f^{-1}(Y) 
\end{cases}
$ where $X$ and $Y$ are two dual outputs. 
\\
\midgrayline
Challenges & (i) Balancing multiple constraints: summarization, neologistic, and algorithmic; (ii) There are limited techniques for neologistic, and algorithmic requirements.  & (i) Involving creative word form, combining words or parts of words in novel ways; (ii) Grammatically correct and pronounceable; (iii) Accurately reflecting the meaning of the original phrase.  & (i) Adhering to controlled elements while maintaining text quality and diversity; (ii) Understanding the semantics of the controlled elements and translating them into appropriate linguistic features. & (i) Ensuring dual dependency; (ii) Capturing the intricate relationships between two different types of text; (iii) Maintaining consistency and coherence across dual outputs.\\ 
\midgrayline
Evaluation metrics & Summarization, neologistic, and algorithmic aspects. &  Creativity, relevance, and impact metrics. & Evaluated based on control adherence and text quality. & Evaluated based on accuracy and coherence between dual texts. \\
\midgrayline
Applications & 
% Branding~\cite{yang-etal-2023-multimodal}, 
Academic~\cite{zhang-tetreault-2019-email}, news recommendation~\cite{cai-etal-2023-generating}, SEO~\cite{tsuruoka-etal-2005-machine}, etc~(\Appendix~\ref{appendix:applications}).  & Search engine optimization~(SEO)~\cite{tsuruoka-etal-2005-machine}  & Attribute-based generation~\cite{saha-etal-2022-countergedi}, debiasing~\cite{dinan-etal-2020-queens}, data to text~\cite{ribeiro-etal-2021-structural}, etc. & Machine translation~(forward and backward)~\cite{he-etal-2016-dual}, Question and answer generation~\cite{tang-etal-2017-question}, etc.  \\
\hline
Unique contributions of \shorttitle &  
\multicolumn{4}{p{ \fourColumnComparisonWidth cm}}{\shorttitle highlights the interplay of summarization requirements, neologistic creativity, and algorithmic precision. Its standout contributions lie in its challenges of novel neologistic and algorithmic demands. The three requirements make it particularly suited for applications where branding, marketing impact, and search engine optimization. } 
\\
\bottomrule
\end{tabular}

==> sections/limitations.tex <==
The study investigates the causal epistemic consistency of cause-effect pairs given one intermediate at a time. However, combinations of fine-grained intermediates can have more complex effects on the causal pair; hence, future work could extend on this work by examining the impact of combinations of intermediates on the causal epistemic consistency.
